Probabilistic Generative Modeling for Procedural Roundabout Generation for Developing Countries

Due to limited resources and fast economic growth, designing optimal transportation road networks with traffic simulation and validation in a cost-effective manner is vital for developing countries, where extensive manual testing is expensive and often infeasible. Current rule-based road design generators lack diversity, a key feature for design robustness. Generative Flow Networks (GFlowNets) learn stochastic policies to sample from an unnormalized reward distribution, thus generating high-quality solutions while preserving their diversity. In this work, we formulate the problem of linking incident roads to the circular junction of a roundabout by a Markov decision process, and we leverage GFlowNets as the Junction-Art road generator. We compare our method with related methods and our empirical results show that our method achieves better diversity while preserving a high validity score.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section 2 (`General formatting instructions') of the tex template (`Formatting Instructions For NeurIPS 2021').}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Abstract and introduction directly reflect the paper's contribution and scope }
    
    
  \item Did you describe the limitations of your work?
     \answerYes{see last paragraph of section 6 of the manuscript }
     
     
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{This study is purely technical and do not involve any social aspects}
    
    
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See section 2 and related appendix}
    
	\item Did you include complete proofs of all theoretical results?
    \answerYes{see appendix}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{see section 2, URL available after double-blind review}
    
    
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{see appendix}
    
    
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{see figures with bar and box plot, error bars and p-val provided}
    
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See appendix}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{ all cited}
    
    
  \item Did you mention the license of the assets?
    \answerYes{}
    
    
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{ new dataset released together with code on github after double-blind review}
    
    
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{ publicly available data used}
    
    
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{ no personally identifiable information included}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> eqns/reward.tex <==
\begin{equation}
\label{reward}
R(roundabout) = 
\left\{
    \begin{array}{lr}
        D(roundabout) & \text{if roundabout is valid} \\
         0 & \text{otherwise }  
    \end{array}
\right\} 
\end{equation}

==> figs/contactPoints.tex <==
\begin{figure}[bt!]
    \centering
    \includegraphics[width=.9\linewidth]{imgs/Road Contact Points.png}
    \caption{For each slots, incident roads can connect to the circular roads in two different manner. They can connect to the start point of the successor circular segment or the end point of the predecessor circular segment.}
    \label{fig:concactPoint}
\end{figure}
